Symmetrizing Cost of Quantum States

We introduce and analyze a task that we call symmetrization, in which a state of a quantum system, associated with a symmetry group, is transformed by a random unitary operation to a symmetric state. Each element of the unitary ensemble is required to be symmetry preserving, in the sense that it keeps the set of symmetric states invariant. We consider an asymptotic limit of infinitely many copies and vanishingly small error, and analyze the symmetrizing cost, that is, the minimum cost of randomness per copy required for symmetrization. We prove that the symmetrizing cost of an arbitrary quantum state is equal to the relative entropy of frameness, thereby providing it with a direct operational meaning.

==> symmetrizing cost/commands.tex <==
\newcommand{\bra}[1]{\mbox{$\left\langle#1\right|$}}
\newcommand{\ket}[1]{\mbox{$\left|#1\right\rangle$}}
\newcommand{\inpro}[2]{\mbox{$\left\langle#1|#2\right\rangle$}}
\newcommand{\outpro}[2]{\mbox{$\ket{#1}\!\bra{#2}$}}
\newcommand{\proj}[1]{\mbox{$\ket{#1}\!\bra{#1}$}}
\newcommand{\kakko}[1]{\mbox{$\left(#1\right)$}}
\newcommand{\proof}{\noindent{\bf Proof.}  }
\newcommand{\ave}[1]{\mbox{$\left\langle#1\right\rangle$}}
\newcommand{\eq}[1]{Eq.(\ref{eq:#1})}
\newcommand{\sect}[1]{Sec.\,\ref{sec:#1}}
\newcommand{\ep}[1]{\noindent{\underline{\bf EP{#1}:}}}
\newcommand{\alg}[1]{\begin{align}#1\end{align}}
\newcommand{\rarrow}{\rightarrow}
\newcommand{\larrow}{\leftarrow}
\newcommand{\ca}[1]{{\mathcal #1}}
\newcommand{\Tr}[2]{{\rm Tr}_{#1}\left[#2\right]}
\newcommand{\bthm}[1]{\begin{thm}\label{thm:#1}}
\newcommand{\ethm}{\end{thm}}
\newcommand{\rthm}[1]{Theorem \ref{thm:#1}}
\newcommand{\blmm}[1]{\begin{lmm}\label{lmm:#1}}
\newcommand{\elmm}{\end{lmm}}
\newcommand{\bdfn}[1]{\begin{dfn}\label{dfn:#1}}
\newcommand{\edfn}{\end{dfn}}
\newcommand{\bprf}{\begin{prf}}
\newcommand{\eprf}{\end{prf}}
\newcommand{\brmk}{\begin{rmk}}
\newcommand{\ermk}{\end{rmk}}
\newcommand{\req}[1]{Equality (\ref{eq:#1})}
\newcommand{\rineq}[1]{Inequality (\ref{eq:#1})}
\newcommand{\QED}{\hfill$\blacksquare$}
\newcommand{\lsec}[1]{\label{sec:#1}}
\newcommand{\rsec}[1]{\ref{sec:#1}}
\newcommand{\aR}{a_{\scalebox{0.45}{$R$}}}
\newcommand{\aL}{a_{\scalebox{0.45}{$L$}}}
\newcommand{\az}{a_{\scalebox{0.45}{$0$}}}
\newcommand{\bR}{b_{\scalebox{0.45}{$R$}}}
\newcommand{\bL}{b_{\scalebox{0.45}{$L$}}}
\newcommand{\bz}{b_{\scalebox{0.45}{$0$}}}
\newcommand{\baR}{{\bar a}_{\scalebox{0.45}{$R$}}}
\newcommand{\baL}{{\bar a}_{\scalebox{0.45}{$L$}}}
\newcommand{\baz}{{\bar a}_{\scalebox{0.45}{$0$}}}
\newcommand{\bbR}{{\bar b}_{\scalebox{0.45}{$R$}}}
\newcommand{\bbL}{{\bar b}_{\scalebox{0.45}{$L$}}}
\newcommand{\bbz}{{\bar b}_{\scalebox{0.45}{$0$}}}

 

==> symmetrizing cost/preferences_ieee.tex <==

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{thm}{ Theorem}
\newtheorem{dfn}[thm]{ Definition}
\newtheorem{lmm}[thm]{ Lemma}
\newtheorem{exa}[thm]{ Example}
\newtheorem{crl}[thm]{ Corollary}
\newtheorem{cjt}[thm]{ Conjecture}
\newtheorem{prp}[thm]{ Proposition}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{prf}{ Proof:}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{skprf}{ Sketch of the proof.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{outprf}{ Outline of the proof.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{prftyp}{ Proof of Theorem \ref{thm:typicalsubspace}.}}

{\theorembodyfont{\normalfont}
\theoremheaderfont{\normalfont\it}
\newtheorem{rmk}{ Remark.}}

\renewcommand{\theprf}{}
\renewcommand{\theprftyp}{}
\renewcommand{\theoutprf}{}
\renewcommand{\thermk}{}



  
